Hypergraph Neural Networks through the Lens of Message Passing: A Common Perspective to Homophily and Architecture Design

Most of the current hypergraph learning methodologies and benchmarking datasets in the hypergraph realm are obtained by lifting procedures from their graph analogs, leading to overshadowing specific characteristics of hypergraphs. This paper attempts to confront some pending questions in that regard: Q1 Can the concept of homophily play a crucial role in Hypergraph Neural Networks (HNNs)? Q2 Is there room for improving current HNN architectures by carefully addressing specific characteristics of higher-order networks? Q3 Do existing datasets provide a meaningful benchmark for HNNs? To address them, we first introduce a novel conceptualization of homophily in higher-order networks based on a Message Passing (MP) scheme, unifying both the analytical examination and the modeling of higher-order networks. Further, we investigate some natural, yet mostly unexplored, strategies for processing higher-order structures within HNNs such as keeping hyperedge-dependent node representations, or performing node/hyperedge stochastic samplings, leading us to the most general MP formulation up to date -MultiSet-, as well as to an original architecture design, MultiSetMixer. Finally, we conduct an extensive set of experiments that contextualize our proposals and successfully provide insights about our inquiries.

==> figures/Edge-homophily.tex <==



\subsection{Figure - $k$-uniform homophily}
Some of the hypergraphs have a lot of different size for hyperedges, here, we report the plots only for some $k$ for each dataset for brevity. All additional plots can be found in the supplementary material's zip files.

\begin{figure}[ht]
    \centering
    \includegraphics[width=1\textwidth]{figures/edge_homophily/cora/0.png}
    \caption{$k$-uniform homophily Cora.}
\end{figure}
\FloatBarrier

\begin{figure}[ht]
    \centering
    \includegraphics[width=1\textwidth]{figures/edge_homophily/cora/1.png}
    \caption{$k$-uniform homophily Cora.}
\end{figure}
\FloatBarrier

\begin{figure}[ht]
    \centering
    \includegraphics[width=1\textwidth]{figures/edge_homophily/cora/2.png}
    \caption{$k$-uniform homophily Cora.}
\end{figure}
\FloatBarrier

\begin{figure}[ht]
    \centering
    \includegraphics[width=1\textwidth]{figures/edge_homophily/CORA_CA/0.png}
    \caption{$k$-uniform homophily CORA-CA.}
\end{figure}
\FloatBarrier

\begin{figure}[ht]
    \centering
    \includegraphics[width=1\textwidth]{figures/edge_homophily/CORA_CA/1.png}
    \caption{$k$-uniform homophily CORA-CA.}
\end{figure}
\FloatBarrier

\begin{figure}[ht]
    \centering
    \includegraphics[width=1\textwidth]{figures/edge_homophily/CORA_CA/2.png}
    \caption{$k$-uniform homophily CORA-CA.}
\end{figure}
\FloatBarrier

\begin{figure}[ht]
    \centering
    \includegraphics[width=1\textwidth]{figures/edge_homophily/DBLP_CA/0.png}
    \caption{$k$-uniform homophily DBLP-CA.}
\end{figure}
\FloatBarrier

\begin{figure}[ht]
    \centering
    \includegraphics[width=1\textwidth]{figures/edge_homophily/DBLP_CA/1.png}
    \caption{$k$-uniform homophily DBLP-CA.}
\end{figure}
\FloatBarrier

\begin{figure}[ht]
    \centering
    \includegraphics[width=1\textwidth]{figures/edge_homophily/DBLP_CA/2.png}
    \caption{$k$-uniform homophily DBLP-CA.}
\end{figure}
\FloatBarrier

\begin{figure}[ht]
    \centering
    \includegraphics[width=1\textwidth]{figures/edge_homophily/ModelNet40/0.png}
    \caption{$k$-uniform homophily ModelNet40.}
\end{figure}
\FloatBarrier


\begin{figure}[ht]
    \centering
    \includegraphics[width=1\textwidth]{figures/edge_homophily/NTU2012/0.png}
    \caption{$k$-uniform homophily NTU2012.}
\end{figure}
\FloatBarrier


\begin{figure}[ht]
    \centering
    \includegraphics[width=1\textwidth]{figures/edge_homophily/pubmed/0.png}
    \caption{$k$-uniform homophily Pubmed.}
\end{figure}
\FloatBarrier

\begin{figure}[ht]
    \centering
    \includegraphics[width=1\textwidth]{figures/edge_homophily/pubmed/1.png}
    \caption{$k$-uniform homophily Pubmed.}
\end{figure}
\FloatBarrier

\begin{figure}[ht]
    \centering
    \includegraphics[width=1\textwidth]{figures/edge_homophily/pubmed/2.png}
    \caption{$k$-uniform homophily Pubmed.}
\end{figure}
\FloatBarrier

\begin{figure}[ht]
    \centering
    \includegraphics[width=1\textwidth]{figures/edge_homophily/zoo/0.png}
    \caption{$k$-uniform homophily ZOO.}
\end{figure}
\FloatBarrier


\begin{figure}[ht]
    \centering
    \includegraphics[width=1\textwidth]{figures/edge_homophily/zoo/1.png}
    \caption{$k$-uniform homophily ZOO.}
\end{figure}
\FloatBarrier

\begin{figure}[ht]
    \centering
    \includegraphics[width=1\textwidth]{figures/edge_homophily/zoo/2.png}
    \caption{$k$-uniform homophily ZOO.}
\end{figure}
\FloatBarrier


==> figures/NODE_HOMO_PLOTS.tex <==
\subsection{Figure - node homophily}
\begin{figure}[ht]
    \centering
    \includegraphics[width=1\textwidth]{figures/node_homophily/cora_node.png}
    \caption{Node Homophily Distribution Scores for Cora.}
    \label{fig:node_homophily_cora }
\end{figure}
\FloatBarrier

\begin{figure}[ht]
    \centering
    \includegraphics[width=1\textwidth]{figures/node_homophily/citeseer_node.png}
    \caption{Node Homophily Distribution Scores for Citeseer.}
    \label{fig:node_homophily_citeseer}
\end{figure}
\FloatBarrier

\begin{figure}[ht]
    \centering
    \includegraphics[width=1\textwidth]{figures/node_homophily/coauthor_cora_node.png}
    \caption{Node Homophily Distribution Scores for CORA-CA.}    \label{fig:node_homophily_coauthor_cora}
\end{figure}
\FloatBarrier


\begin{figure}[ht]
    \centering
    \includegraphics[width=1\textwidth]{figures/node_homophily/coauthor_dblp_node.png}
    \caption{Node Homophily Distribution Scores for DBLP-CA.}
    \label{fig:node_homophily_coauthor_dblp}
\end{figure}
\FloatBarrier

\begin{figure}[ht]
    \centering
    \includegraphics[width=1\textwidth]{figures/node_homophily/NTU2012_node.png}
    \caption{ Node Homophily Distribution Scores for NTU2012.}
    \label{fig:node_homophily_ntu2012}
\end{figure}
\FloatBarrier
%\newpage

\begin{figure}[ht]
    \centering
    \includegraphics[width=1\textwidth]{figures/node_homophily/ModelNet40_node.png}
    \caption{Node Homophily Distribution Scores for ModelNet40.}
    \label{fig:node_homophily_modelnet40}
\end{figure}
\FloatBarrier


\begin{figure}[ht]
    \centering
    \includegraphics[width=1\textwidth]{figures/node_homophily/Mushroom_node.png}
    \caption{ Node Homophily Distribution Scores for Mushroom.}
    \label{fig:node_homophily_mushroom}
\end{figure}
\FloatBarrier

\begin{figure}[ht]
    \centering
    \includegraphics[width=1\textwidth]{figures/node_homophily/20newsW100_node.png}
    \caption{Node Homophily Distribution Scores for 20NewsW100.}
    %\label{fig:node_homophily_20News}
\end{figure}
\FloatBarrier


\begin{figure}[ht]
    \centering
    \includegraphics[width=1\textwidth]{figures/node_homophily/zoo_node.png}
    \caption{Node Homophily Distribution Scores for ZOO.}
   % \label{fig:node_homophily_20News}
\end{figure}
\FloatBarrier



==> tables/avr_ranking.tex <==
\begin{table}[ht]
\caption{Average Rankings for All Splits and Mean Average Ranking.}
 \label{table:results_average_ranking}
\begin{adjustbox}{width=\textwidth} 
%\begin{center}
\centering
\begin{tabular}{c| c c c c c c c c c c c c c c c c }
            
\hline

Model &  AllSetTransformer &  UniGCNII &  HCHA &  HNHN &  HGNN &  AllDeepSets &  MultiSetMixer &   HAN &  Transformer  Classic &  MLP  HP &  MLP  classic &   CEGAT &   CEGCN &  MMLP  HP &    MLP &  HyperGCN \\
\midrule
0.1 &               3.75 &      3.35 &  4.85 &  7.45 &  5.05 &         5.85 &         6.700 &  6.80 &                9.320 &  10.100 &       10.090 &  10.670 &  11.000 &   11.880 &  12.05 &     13.70 \\
0.2 &               3.35 &      3.50 &  5.50 &  7.20 &  5.70 &         6.25 &         6.700 &  7.25 &                9.270 &  10.300 &       10.500 &  11.000 &  11.890 &   12.000 &  12.70 &     14.10 \\
0.3 &               3.30 &      3.65 &  6.40 &  5.50 &  6.70 &         6.55 &         6.900 &  7.60 &                8.680 &  10.400 &       10.270 &  11.280 &  11.780 &   12.120 &  13.00 &     14.20 \\
0.4 &               3.15 &      3.55 &  6.50 &  5.30 &  6.50 &         6.40 &         6.700 &  8.45 &                8.360 &   9.800 &        9.770 &  11.000 &  12.170 &   12.880 &  12.80 &     14.00 \\
0.5 &               2.85 &      4.15 &  6.95 &  5.05 &  7.05 &         6.10 &         6.270 &  8.60 &                8.500 &   9.640 &        9.910 &  11.330 &  12.000 &   11.890 &  12.90 &     14.30 \\
avg &               3.28 &      3.64 &  6.04 &  6.10 &  6.20 &         6.23 &         6.654 &  7.74 &                8.826 &  10.048 &       10.108 &  11.056 &  11.768 &   12.154 &  12.69 &     14.06 \\

\hline
\end{tabular}

\end{adjustbox}
\end{table}
\FloatBarrier


==> tables/homophily_absolute_vals.tex <==
\begin{table}[ht]
\caption{Absolute Homophily}
\label{table:absolute homophily values}
\begin{adjustbox}{width=\textwidth} 
\centering
\begin{tabular}{l|rrrrrrrrrr}
\toprule
& Cora & Citeseer & Pubmed & CORA-CA & DBLP-CA & Mushroom & NTU2012 & ModelNet40 & 20Newsgroups & ZOO \\
\midrule
CE Homophily & 89.74 & 89.32 & 95.24 & 80.26 & 86.88 & 82.88 & 75.25 & 85.33 & 46.07 & 24.07 \\
$h^0_{v}$ & 84.10 & 78.25 & 82.05 & 80.81 & 88.86 & 91.13 & 81.26 & 88.05 & 53.24 & 42.16 \\
$h^1_{v}$ & 78.08 & 74.18 & 75.73 & 76.51 & 86.01 & 85.79 & 74.78 & 84.41 & 41.95 & 29.42 \\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table}
\FloatBarrier

==> tables/not_used.tex <==
\begin{table}[ht]
\caption{Adjust connectivity. Test accuracy in \% averaged over 15 splits.}
 \label{table: kmeans_exp_main}
\begin{adjustbox}{width=\textwidth} 

\centering

\begin{tabular}{c| c| c c c c c c c c c c c }
            
\hline
        
Model & Type & Cora & Citeseer & Pubmed & CORA-CA & DBLP-CA & Mushroom & NTU2012 & ModelNet40 & 20Newsgroups & ZOO & avg. ranking \\

\hline

 & Label Based & \cellcolor{gray!25} \textbf{82.24 ± 1.12} & \cellcolor{gray!25} \textbf{75.65 ± 1.57} & \cellcolor{gray!25} \textbf{90.49 ± 0.40} & \cellcolor{gray!25} \textbf{91.12 ± 0.92} & \cellcolor{gray!25} \textbf{96.59 ± 0.17} & \cellcolor{gray!25} \textbf{99.96 ± 0.04} & \cellcolor{gray!25} \textbf{93.13 ± 1.29} & \cellcolor{gray!25} \textbf{99.52 ± 0.11} & \cellcolor{gray!25} \textbf{99.79 ± 0.13} & \cellcolor{gray!25} \textbf{91.54 ± 7.24} & \cellcolor{gray!25} \textbf{1.05} \\
AllDeepSets& $k$-means  & 75.20 ± 1.11 & 70.87 ± 1.54 & 88.96 ± 0.48 & 79.59 ± 1.42 & 89.75 ± 0.25 & \cellcolor{blue!25} 99.94 ± 0.09 & 84.23 ± 1.50 & 97.17 ± 0.13 & 81.18 ± 0.54 & \cellcolor{blue!25} 86.92 ± 7.73 & 2.80 \\
 & Original & 77.11 ± 1.00 & 70.67 ± 1.42 & 89.04 ± 0.45 & 82.23 ± 1.46 & 91.34 ± 0.27 & \cellcolor{gray!25} \textbf{99.96 ± 0.05} & 86.49 ± 1.86 & 96.70 ± 0.25 & 81.19 ± 0.49 & \cellcolor{blue!25} 89.10 ± 7.00 & 2.15 \\

\hline
 & Label Based & \cellcolor{gray!25} \textbf{83.43 ± 1.36} & \cellcolor{gray!25} \textbf{76.45 ± 1.43} & \cellcolor{gray!25} \textbf{90.19 ± 0.42} & \cellcolor{gray!25} \textbf{91.71 ± 0.89} & \cellcolor{gray!25} \textbf{96.75 ± 0.16} & \cellcolor{gray!25} \textbf{99.96 ± 0.05} & \cellcolor{gray!25} \textbf{94.81 ± 1.04} & \cellcolor{gray!25} \textbf{99.68 ± 0.09} & \cellcolor{gray!25} \textbf{99.93 ± 0.03} & \cellcolor{gray!25} \textbf{94.10 ± 6.91} & \cellcolor{gray!25} \textbf{1.05} \\
AllSetTransformer & $k$-means  & 77.14 ± 1.46 & 72.83 ± 1.07 & 88.60 ± 0.41 & 81.92 ± 1.35 & 89.79 ± 0.30 & \cellcolor{gray!25} \textbf{99.96 ± 0.06} & 87.95 ± 1.28 & 97.29 ± 0.20 & 81.58 ± 0.55 & \cellcolor{blue!25} 88.72 ± 7.69 & 2.75 \\
 & Original & 79.54 ± 1.02 & 72.52 ± 0.88 & 88.74 ± 0.51 & 84.43 ± 1.14 & 91.61 ± 0.19 & \cellcolor{blue!25} 99.95 ± 0.05 & 88.22 ± 1.42 & 98.00 ± 0.12 & 81.59 ± 0.59 & \cellcolor{blue!25} 91.03 ± 7.31 & 2.20 \\
 
\hline

 & Label Based & \cellcolor{gray!25} \textbf{83.70 ± 1.02} & \cellcolor{gray!25} \textbf{77.50 ± 1.53} & \cellcolor{gray!25} \textbf{90.08 ± 0.42} & \cellcolor{gray!25} \textbf{91.28 ± 0.97} & \cellcolor{gray!25} \textbf{96.68 ± 0.14} & \cellcolor{gray!25} \textbf{99.95 ± 0.05} & \cellcolor{gray!25} \textbf{94.03 ± 1.24} & \cellcolor{gray!25} \textbf{99.30 ± 0.14} & OOM & \cellcolor{gray!25} \textbf{95.00 ± 7.08} & \cellcolor{gray!25} \textbf{1.00} \\
CEGCN & $k$-means  & 75.89 ± 1.53 & 72.07 ± 1.18 & 87.13 ± 0.51 & 76.43 ± 1.41 & 86.76 ± 0.24 & 94.84 ± 0.47 & 85.34 ± 1.71 & 95.77 ± 0.31 & OOM & 73.72 ± 7.89 & 2.44 \\
 & Original & 77.03 ± 1.31 & 70.87 ± 1.19 & 87.01 ± 0.62 & 77.55 ± 1.65 & 88.12 ± 0.25 & 94.91 ± 0.44 & 80.90 ± 1.74 & 90.04 ± 0.47 & OOM & 49.23 ± 6.81 & 2.56 \\
% \hline

%  & Label Based & \cellcolor{gray!25} \textbf{84.06 ± 1.08} & \cellcolor{gray!25} \textbf{77.12 ± 1.37} & \cellcolor{gray!25} \textbf{88.81 ± 0.43} & \cellcolor{gray!25} \textbf{92.77 ± 0.73} & \cellcolor{gray!25} \textbf{96.70 ± 0.12} & \cellcolor{gray!25} \textbf{99.96 ± 0.06} & \cellcolor{gray!25} \textbf{95.21 ± 1.27} & \cellcolor{gray!25} \textbf{99.67 ± 0.09} & \cellcolor{gray!25} \textbf{99.93 ± 0.04} & \cellcolor{gray!25} \textbf{94.61 ± 6.97} & \cellcolor{gray!25} \textbf{1.00} \\
% HCHA & $k$-means  & 77.51 ± 1.41 & 72.62 ± 1.33 & 86.89 ± 0.48 & 81.19 ± 1.31 & 89.42 ± 0.29 & 99.56 ± 0.27 & 87.62 ± 1.33 & 96.98 ± 0.15 & 80.58 ± 0.57 & 84.10 ± 9.83 & 2.60 \\
%  & Original & 79.53 ± 1.33 & 72.57 ± 1.06 & 86.97 ± 0.55 & 83.53 ± 1.12 & 91.21 ± 0.28 & 98.94 ± 0.54 & 86.60 ± 1.96 & 94.50 ± 0.33 & 80.75 ± 0.53 & \cellcolor{blue!25} 89.23 ± 6.81 & 2.40 \\



\hline
 & Label Based & \cellcolor{gray!25} \textbf{82.59 ± 0.94} & \cellcolor{gray!25} \textbf{76.14 ± 1.03} & \cellcolor{gray!25} \textbf{88.35 ± 0.59} & \cellcolor{gray!25} \textbf{90.86 ± 0.67} & \cellcolor{gray!25} \textbf{96.38 ± 0.22} & \cellcolor{gray!25} \textbf{99.97 ± 0.04} & \cellcolor{gray!25} \textbf{93.72 ± 1.00} & \cellcolor{gray!25} \textbf{99.56 ± 0.12} & \cellcolor{gray!25} \textbf{99.85 ± 0.06} & \cellcolor{gray!25} \textbf{91.79 ± 6.90} & \cellcolor{gray!25} \textbf{1.05} \\

MultiSetMixer & kmeans based & 76.78 ± 1.15 & 73.10 ± 1.18 & 85.84 ± 0.59 & 80.06 ± 1.45 & 88.54 ± 0.27 & \cellcolor{gray!25} \textbf{99.97 ± 0.05} & 87.75 ± 1.09 & 96.94 ± 0.26 & 81.14 ± 0.47 & \cellcolor{blue!25} 85.41 ± 6.77 & 2.55 \\

& Original & 79.38 ± 1.08 & 72.79 ± 1.12 & 85.71 ± 0.49 & 82.62 ± 1.20 & 89.87 ± 0.29 & 95.85 ± 3.21 & 88.73 ± 1.29 & 98.15 ± 0.19 & 87.83 ± 2.68 & 78.67 ± 9.08 & 2.40 \\





\hline




\end{tabular}

\end{adjustbox}
\end{table}



==> tables/not_used2.tex <==
\begin{table*}[ht]


\caption{Drop connectivity. Test accuracy in \% averaged over 15 splits.}
 \label{table: quantile_exp_main}
\begin{adjustbox}{width=\textwidth} 

\centering

\begin{tabular}{c| c| c c c c c c c c c c c }
            
\hline
        
Model & Type & Cora & Citeseer & Pubmed & CORA-CA & DBLP-CA & Mushroom & NTU2012 & ModelNet40 & 20Newsgroups & ZOO & avg. ranking \\
\hline
\multirow[c]{10}{*}{\rotatebox[origin=c]{90}{AllSetTransformer}} & Original & \cellcolor{gray!25} \textbf{79.54 ± 1.02} & \cellcolor{blue!25} 72.52 ± 0.88 & \cellcolor{gray!25} \textbf{88.74 ± 0.51} & \cellcolor{gray!25} \textbf{84.43 ± 1.14} & \cellcolor{gray!25} \textbf{91.61 ± 0.19} & \cellcolor{blue!25} 99.95 ± 0.05 & \cellcolor{gray!25} \textbf{88.22 ± 1.42} & \cellcolor{gray!25} \textbf{98.00 ± 0.12} & \cellcolor{blue!25} 81.59 ± 0.59 & \cellcolor{blue!25} 91.03 ± 7.31 & \cellcolor{gray!25} \textbf{1.95} \\
 & Random 25\% & \cellcolor{blue!25} 79.11 ± 0.99 & \cellcolor{gray!25} \textbf{72.75 ± 1.14} & \cellcolor{blue!25} 88.67 ± 0.47 & 82.36 ± 1.38 & 90.61 ± 0.29 & \cellcolor{blue!25} 99.94 ± 0.09 & \cellcolor{blue!25} 87.50 ± 1.36 & \cellcolor{blue!25} 97.98 ± 0.17 & \cellcolor{gray!25} \textbf{81.70 ± 0.52} & \cellcolor{blue!25} 89.87 ± 7.66 & 3.10 \\
 & Random 50\% & 77.77 ± 1.34 & \cellcolor{blue!25} 72.21 ± 1.25 & \cellcolor{blue!25} 88.50 ± 0.45 & 79.73 ± 1.58 & 89.46 ± 0.27 & \cellcolor{blue!25} 99.96 ± 0.04 & \cellcolor{blue!25} 87.34 ± 1.55 & 97.83 ± 0.17 & \cellcolor{blue!25} 81.55 ± 0.66 & \cellcolor{blue!25} 89.49 ± 6.30 & 5.85 \\
 & Random 75\% & 76.92 ± 1.20 & \cellcolor{blue!25} 72.40 ± 1.22 & \cellcolor{blue!25} 88.54 ± 0.47 & 77.88 ± 1.74 & 87.73 ± 0.32 & 99.76 ± 0.15 & 86.31 ± 1.34 & 97.52 ± 0.20 & \cellcolor{blue!25} 81.46 ± 0.62 & \cellcolor{blue!25} 87.69 ± 6.09 & 8.10 \\
 & Retention 25\% & \cellcolor{blue!25} 79.19 ± 1.11 & \cellcolor{blue!25} 72.49 ± 0.86 & \cellcolor{blue!25} 88.73 ± 0.40 & \cellcolor{blue!25} 83.58 ± 1.30 & 91.18 ± 0.17 & \cellcolor{blue!25} 99.93 ± 0.09 & \cellcolor{blue!25} 87.21 ± 1.58 & 97.82 ± 0.17 & \cellcolor{blue!25} 81.63 ± 0.48 & \cellcolor{blue!25} 86.92 ± 7.18 & 4.10 \\
 & Retention 50\% & 78.16 ± 0.98 & \cellcolor{blue!25} 72.55 ± 1.13 & \cellcolor{blue!25} 88.70 ± 0.37 & 82.90 ± 1.15 & 90.80 ± 0.22 & 99.89 ± 0.18 & 86.67 ± 1.64 & 97.36 ± 0.21 & \cellcolor{blue!25} 81.61 ± 0.49 & \cellcolor{blue!25} 88.08 ± 7.51 & 5.20 \\
 & Retention 75\% & 77.38 ± 1.35 & \cellcolor{blue!25} 72.43 ± 0.98 & \cellcolor{blue!25} 88.71 ± 0.39 & 81.07 ± 1.20 & 89.83 ± 0.25 & \cellcolor{gray!25} \textbf{99.97 ± 0.04} & 85.58 ± 1.70 & 97.27 ± 0.22 & \cellcolor{blue!25} 81.58 ± 0.48 & \cellcolor{blue!25} 88.97 ± 6.91 & 5.80 \\
 & Trimming 25\% & 75.83 ± 1.31 & \cellcolor{blue!25} 72.39 ± 1.50 & \cellcolor{blue!25} 88.40 ± 0.45 & 76.51 ± 1.35 & 86.38 ± 0.32 & 99.84 ± 0.13 & \cellcolor{blue!25} 86.88 ± 1.66 & 97.10 ± 0.24 & \cellcolor{blue!25} 81.55 ± 0.55 & \cellcolor{gray!25} \textbf{93.08 ± 7.79} & 8.05 \\
 & Trimming 50\% & 77.37 ± 1.17 & \cellcolor{blue!25} 72.32 ± 1.30 & \cellcolor{blue!25} 88.49 ± 0.40 & 77.41 ± 1.73 & 87.03 ± 0.27 & 99.91 ± 0.12 & \cellcolor{blue!25} 86.86 ± 1.53 & 97.86 ± 0.21 & \cellcolor{blue!25} 81.45 ± 0.50 & \cellcolor{blue!25} 89.74 ± 8.53 & 7.50 \\
 & Trimming 75\% & 78.15 ± 1.11 & \cellcolor{blue!25} 72.67 ± 1.00 & \cellcolor{blue!25} 88.48 ± 0.39 & 78.91 ± 1.54 & 88.55 ± 0.26 & 99.92 ± 0.09 & \cellcolor{blue!25} 87.68 ± 1.56 & \cellcolor{blue!25} 97.90 ± 0.23 & \cellcolor{blue!25} 81.41 ± 0.61 & \cellcolor{blue!25} 91.03 ± 7.17 & 5.35 \\

\hline

\multirow[c]{10}{*}{\rotatebox[origin=c]{90}{CEGCN}} & Original & \cellcolor{gray!25} \textbf{77.03 ± 1.31} & \cellcolor{blue!25} 70.87 ± 1.19 & \cellcolor{blue!25} 87.01 ± 0.62 & \cellcolor{gray!25} \textbf{77.55 ± 1.65} & \cellcolor{gray!25} \textbf{88.12 ± 0.25} & 94.91 ± 0.44 & 80.90 ± 1.74 & 90.04 ± 0.47 & OOM & 49.23 ± 6.81 & 4.61 \\
 & Random 25\% & \cellcolor{blue!25} 76.08 ± 1.55 & \cellcolor{blue!25} 71.35 ± 1.44 & \cellcolor{blue!25} 86.89 ± 0.59 & \cellcolor{blue!25} 76.51 ± 1.53 & 87.01 ± 0.39 & 93.11 ± 0.46 & 80.68 ± 1.86 & 90.36 ± 0.46 & OOM & 49.74 ± 6.22 & 6.22 \\
 & Random 50\% & 75.55 ± 1.63 & \cellcolor{blue!25} 71.42 ± 1.60 & 86.70 ± 0.48 & 75.27 ± 1.22 & 86.24 ± 0.35 & 93.28 ± 0.61 & 80.63 ± 1.78 & 90.69 ± 0.54 & OOM & 56.92 ± 7.24 & 6.33 \\
 & Random 75\% & 75.34 ± 1.62 & \cellcolor{blue!25} 71.73 ± 1.90 & \cellcolor{blue!25} 86.97 ± 0.51 & 74.53 ± 1.56 & 85.36 ± 0.26 & 93.01 ± 0.45 & 80.56 ± 1.76 & \cellcolor{blue!25} 91.91 ± 0.54 & OOM & 63.20 ± 5.59 & 6.33 \\
 & Retention 25\% & \cellcolor{blue!25} 76.12 ± 1.58 & \cellcolor{blue!25} 70.87 ± 1.42 & \cellcolor{blue!25} 86.94 ± 0.56 & \cellcolor{blue!25} 76.98 ± 1.53 & \cellcolor{blue!25} 87.90 ± 0.29 & 94.94 ± 0.48 & 79.20 ± 1.42 & 90.59 ± 0.59 & OOM & 49.87 ± 7.59 & 5.50 \\
 & Retention 50\% & 75.43 ± 1.28 & \cellcolor{blue!25} 70.83 ± 1.52 & \cellcolor{blue!25} 86.95 ± 0.54 & \cellcolor{blue!25} 76.87 ± 1.49 & 87.58 ± 0.28 & 94.97 ± 0.40 & 78.53 ± 1.90 & 90.09 ± 0.56 & OOM & 45.77 ± 6.88 & 6.89 \\
 & Retention 75\% & 75.53 ± 1.25 & \cellcolor{blue!25} 71.72 ± 1.42 & \cellcolor{blue!25} 87.11 ± 0.53 & \cellcolor{blue!25} 76.36 ± 1.42 & 87.03 ± 0.28 & 94.74 ± 0.39 & 79.82 ± 1.41 & \cellcolor{gray!25} \textbf{92.29 ± 0.46} & OOM & 40.38 ± 5.42 & 5.44 \\
 & Trimming 25\% & 75.58 ± 1.56 & \cellcolor{gray!25} \textbf{72.26 ± 1.52} & \cellcolor{gray!25} \textbf{87.36 ± 0.51} & 74.84 ± 1.31 & 84.97 ± 0.31 & \cellcolor{gray!25} \textbf{99.60 ± 0.11} & \cellcolor{gray!25} \textbf{83.10 ± 1.69} & \cellcolor{blue!25} 91.85 ± 0.42 & OOM & \cellcolor{gray!25} \textbf{87.69 ± 7.31} & \cellcolor{gray!25} \textbf{3.44} \\
 & Trimming 50\% & \cellcolor{blue!25} 76.57 ± 1.47 & \cellcolor{blue!25} 71.81 ± 1.44 & \cellcolor{blue!25} 87.07 ± 0.55 & 74.66 ± 1.68 & 85.24 ± 0.33 & \cellcolor{blue!25} 99.54 ± 0.18 & 80.72 ± 1.64 & 90.64 ± 0.54 & OOM & 71.28 ± 6.60 & 4.00 \\
 & Trimming 75\% & \cellcolor{blue!25} 76.53 ± 1.50 & \cellcolor{blue!25} 71.45 ± 1.45 & 86.75 ± 0.54 & 74.56 ± 1.32 & 85.56 ± 0.33 & 99.14 ± 0.23 & 80.38 ± 1.91 & 90.06 ± 0.37 & OOM & 58.46 ± 7.17 & 6.22 \\

% \hline

% \multirow[c]{10}{*}{\rotatebox[origin=c]{90}{HCHA}} & Original & \cellcolor{gray!25} \textbf{79.53 ± 1.33} & \cellcolor{gray!25} \textbf{72.57 ± 1.06} & \cellcolor{gray!25} \textbf{86.97 ± 0.55} & \cellcolor{gray!25} \textbf{83.53 ± 1.12} & \cellcolor{gray!25} \textbf{91.21 ± 0.28} & 98.94 ± 0.54 & \cellcolor{gray!25} \textbf{86.60 ± 1.96} & 94.50 ± 0.33 & \cellcolor{gray!25} \textbf{80.75 ± 0.53} & \cellcolor{blue!25} 89.23 ± 6.81 & \cellcolor{gray!25} \textbf{2.40} \\
%  & Random 25\% & \cellcolor{blue!25} 78.74 ± 1.30 & \cellcolor{blue!25} 72.33 ± 1.28 & \cellcolor{blue!25} 86.84 ± 0.56 & 81.98 ± 1.34 & 90.09 ± 0.35 & 98.55 ± 0.55 & \cellcolor{blue!25} 85.94 ± 1.76 & 94.78 ± 0.28 & 80.16 ± 0.46 & \cellcolor{blue!25} 89.10 ± 6.71 & 4.30 \\
%  & Random 50\% & 77.65 ± 1.46 & \cellcolor{blue!25} 72.11 ± 1.42 & \cellcolor{blue!25} 86.67 ± 0.48 & 79.23 ± 1.41 & 88.88 ± 0.35 & 98.61 ± 0.48 & \cellcolor{blue!25} 85.32 ± 1.75 & 95.17 ± 0.28 & 79.68 ± 0.50 & \cellcolor{blue!25} 87.56 ± 6.97 & 6.60 \\
%  & Random 75\% & 76.56 ± 1.60 & \cellcolor{blue!25} 72.23 ± 1.33 & \cellcolor{blue!25} 86.72 ± 0.56 & 77.11 ± 1.28 & 87.07 ± 0.34 & 98.59 ± 0.76 & \cellcolor{blue!25} 84.88 ± 1.44 & \cellcolor{gray!25} \textbf{95.57 ± 0.34} & 79.49 ± 0.43 & 82.18 ± 6.58 & 7.30 \\
%  & Retention 25\% & \cellcolor{blue!25} 79.09 ± 1.25 & \cellcolor{blue!25} 72.29 ± 1.17 & \cellcolor{blue!25} 86.95 ± 0.52 & \cellcolor{blue!25} 83.06 ± 1.09 & 90.63 ± 0.25 & 98.82 ± 0.50 & \cellcolor{blue!25} 85.56 ± 1.66 & 94.73 ± 0.34 & \cellcolor{blue!25} 80.27 ± 0.44 & \cellcolor{blue!25} 86.03 ± 5.20 & 3.85 \\
%  & Retention 50\% & 77.77 ± 1.38 & \cellcolor{blue!25} 72.20 ± 1.20 & \cellcolor{blue!25} 86.82 ± 0.48 & 82.16 ± 1.27 & 90.17 ± 0.29 & 98.22 ± 0.28 & \cellcolor{blue!25} 84.80 ± 1.79 & 94.54 ± 0.22 & 79.96 ± 0.44 & 75.77 ± 6.86 & 6.70 \\
%  & Retention 75\% & 77.05 ± 1.53 & \cellcolor{blue!25} 72.37 ± 1.20 & \cellcolor{blue!25} 86.79 ± 0.47 & 80.79 ± 0.95 & 88.97 ± 0.24 & 97.62 ± 0.30 & 84.35 ± 1.65 & 95.21 ± 0.30 & 79.40 ± 0.52 & 84.36 ± 6.77 & 6.70 \\
%  & Trimming 25\% & 75.68 ± 1.21 & \cellcolor{blue!25} 72.15 ± 1.72 & \cellcolor{blue!25} 86.83 ± 0.47 & 75.94 ± 1.35 & 85.85 ± 0.40 & \cellcolor{gray!25} \textbf{99.87 ± 0.11} & \cellcolor{blue!25} 85.60 ± 1.92 & 95.02 ± 0.26 & \cellcolor{blue!25} 80.66 ± 0.56 & \cellcolor{gray!25} \textbf{91.92 ± 7.10} & 5.50 \\
%  & Trimming 50\% & 77.76 ± 1.28 & \cellcolor{blue!25} 72.10 ± 1.49 & \cellcolor{blue!25} 86.96 ± 0.48 & 77.26 ± 1.17 & 86.57 ± 0.36 & \cellcolor{blue!25} 99.84 ± 0.11 & 84.58 ± 1.37 & 94.73 ± 0.28 & 80.18 ± 0.60 & 83.08 ± 8.72 & 6.45 \\
%  & Trimming 75\% & \cellcolor{blue!25} 78.38 ± 1.30 & \cellcolor{blue!25} 72.22 ± 1.12 & \cellcolor{blue!25} 86.81 ± 0.53 & 78.82 ± 0.95 & 88.09 ± 0.27 & 99.73 ± 0.18 & \cellcolor{blue!25} 86.05 ± 1.60 & 94.61 ± 0.27 & 80.02 ± 0.57 & \cellcolor{blue!25} 89.36 ± 8.49 & 5.20 \\

\hline

\multirow[c]{10}{*}{\rotatebox[origin=c]{90}{MultiSetMixer}} & Original & \cellcolor{gray!25} \textbf{79.38 ± 1.08} & \cellcolor{gray!25} \textbf{72.79 ± 1.12} & 85.71 ± 0.49 & \cellcolor{gray!25} \textbf{82.62 ± 1.20} & \cellcolor{gray!25} \textbf{89.87 ± 0.29} & 95.85 ± 3.21 & \cellcolor{gray!25} \textbf{88.73 ± 1.29} & \cellcolor{gray!25} \textbf{98.15 ± 0.19} & \cellcolor{blue!25} 87.83 ± 2.68 & 78.67 ± 9.08 & \cellcolor{gray!25} \textbf{2.75} \\
 & Random 25\% & \cellcolor{blue!25} 78.63 ± 1.30 & \cellcolor{blue!25} 72.37 ± 1.50 & 85.71 ± 0.55 & 81.18 ± 1.16 & 89.11 ± 0.31 & 93.80 ± 4.69 & \cellcolor{blue!25} 87.92 ± 1.50 & \cellcolor{blue!25} 98.01 ± 0.19 & 76.65 ± 1.76 & 77.60 ± 9.00 & 4.75 \\
 & Random 50\% & 77.66 ± 1.18 & \cellcolor{blue!25} 72.24 ± 1.42 & 85.92 ± 0.45 & 78.51 ± 1.58 & 88.13 ± 0.34 & 94.36 ± 3.79 & 86.22 ± 2.01 & 97.92 ± 0.13 & 74.36 ± 1.23 & 75.53 ± 14.10 & 6.40 \\
 & Random 75\% & 76.59 ± 1.27 & \cellcolor{blue!25} 72.12 ± 1.43 & 86.10 ± 0.53 & 76.91 ± 1.43 & 86.42 ± 0.42 & 98.74 ± 0.90 & 85.31 ± 1.64 & 97.48 ± 0.21 & 76.53 ± 0.75 & 58.75 ± 17.97 & 7.25 \\
 & Retention 25\% & \cellcolor{blue!25} 78.99 ± 1.00 & \cellcolor{blue!25} 72.12 ± 1.28 & 85.73 ± 0.44 & \cellcolor{blue!25} 82.01 ± 1.56 & \cellcolor{blue!25} 89.61 ± 0.33 & 97.18 ± 2.01 & 86.96 ± 1.62 & 97.95 ± 0.19 & \cellcolor{gray!25} \textbf{88.17 ± 2.51} & \cellcolor{blue!25} 80.15 ± 8.87 & 3.85 \\
 & Retention 50\% & 77.88 ± 1.28 & \cellcolor{blue!25} 72.32 ± 1.36 & 85.89 ± 0.52 & 80.85 ± 1.14 & 89.24 ± 0.31 & 97.72 ± 1.42 & 84.56 ± 1.97 & 97.39 ± 0.24 & 85.04 ± 2.06 & 76.31 ± 12.45 & 5.20 \\
 & Retention 75\% & 77.44 ± 1.32 & \cellcolor{blue!25} 72.18 ± 1.32 & 85.93 ± 0.54 & 78.67 ± 1.32 & 87.86 ± 0.35 & 94.75 ± 3.86 & 83.94 ± 1.79 & 97.00 ± 0.26 & 84.65 ± 1.52 & 67.06 ± 18.55 & 7.10 \\
 & Trimming 25\% & 75.54 ± 1.17 & \cellcolor{blue!25} 72.57 ± 1.45 & \cellcolor{gray!25} \textbf{87.26 ± 0.38} & 76.30 ± 1.11 & 85.57 ± 0.34 & \cellcolor{gray!25} \textbf{99.97 ± 0.03} & 83.19 ± 1.55 & 96.87 ± 0.29 & 78.80 ± 0.52 & \cellcolor{gray!25} \textbf{88.51 ± 9.76} & 6.00 \\
 & Trimming 50\% & 76.91 ± 1.18 & \cellcolor{blue!25} 72.30 ± 1.63 & 86.79 ± 0.53 & 77.54 ± 1.44 & 86.16 ± 0.33 & 99.91 ± 0.13 & 84.20 ± 1.75 & 97.70 ± 0.27 & 72.70 ± 0.88 & 69.83 ± 14.25 & 6.60 \\
 & Trimming 75\% & 78.06 ± 1.16 & \cellcolor{blue!25} 72.53 ± 1.30 & 86.45 ± 0.57 & 79.03 ± 1.16 & 87.83 ± 0.29 & 98.49 ± 0.61 & 86.59 ± 1.58 & 97.86 ± 0.24 & 61.17 ± 1.32 & 76.08 ± 10.14 & 5.10 \\

\hline

\end{tabular}

\end{adjustbox}
\end{table*}

